A Hybrid Channel Model based on WINNER for Vehicle-to-X Application

V2V and V2I channel modeling became recently more of interest. To provide realistic radio channels either expensive measurements or complex ray tracing simulations are mostly used. Stochastic channel models are of low complexity but do not offer that deterministic repeatable realism. Based on the WINNER channel model and a simple single path model, a hybrid model has been developed. The concept relies on a layered structure featuring high flexibility and scalability.

==> Sections/Acknowledgments.tex <==
\section*{Acknowledgments}

